Latency-Reliability Tradeoffs for State Estimation

The emerging interest in low-latency high-reliability applications, such as connected vehicles, necessitates a new abstraction between communication and control. Thanks to advances in cyber-physical systems over the past decades, we understand this interface for classical bit-rate models of channels as well as packet-loss-type channels. This work proposes a new abstraction characterized as a tradeoff curve between latency, reliability and rate. Our aim is to understand: Do we (control engineers) prefer faster but less reliable communications (with shorter codes), or slower but more reliable communications (with longer codes)? In this paper we examine the tradeoffs between latency and reliability for the problem of estimating dynamical systems over communication channels. Employing different latency-reliability curves derived from practical coding schemes, we develop a co-design methodology, i.e., select the code length depending on the system dynamics to optimize system performance.

==> abstraction.tex <==

\begin{tikzpicture}[x=0.5cm,y=0.5cm,z=0.3cm,>=stealth]
% The axes
\draw[thick, ->] (xyz cs:x=0) -- (xyz cs:x=13.5) node[above, ] {\huge  \textbf{Rate}};
\draw[thick, ->] (xyz cs:y=0) -- (xyz cs:y=13.5) node[right] {\huge \textbf{Latency}};
\draw[thick, ->] (xyz cs:z=0) -- (xyz cs:z=-13.5) node[above]  {\huge \textbf{Reliability}};

%\draw[dashed, ->] (xyz cs:x=0, y=0, z=0) -- (xyz cs:x=-4, y=12, z=-5.5) node[above] {\huge {\textbf{Uncertainty}}};

\node[align=center, below] at (8,0) (ori) { \Large Date-rate\\ \Large Abstraction};


\node[align=center,right] at (0,0,-8) (ori) {\Large Packet-drop\\ \Large Abstraction};

\node[align=center, right,red] at (0,8,0) (ori) {\Large  
};


\draw[fill=gray!40, opacity=0.2] plot[smooth, samples=100, domain=1:e] (0,0,0) --(0,0,-13) -- (13,0,-13) -- (13,0,0);


\end{tikzpicture}



==> channel_model_new1.tex <==


\tikzstyle{block} = [draw,rectangle,thick,minimum height=1cm,minimum width=1cm,fill=NavyBlue!60, text=white ]
\tikzstyle{connector} = [->,thick]

\begin{tikzpicture}
 \small
    % node placement with matrix library: 5x4 array
    \matrix[ampersand replacement=\&, row sep=0.35cm, column sep=0.20cm] {
    	\node[block] (plant) {\begin{tabular}{c} Plant\\$x_k$ \end{tabular}};
    
    \node[minimum width = 0.0cm] (){};\& 	
    \node[block] (sensor) {\begin{tabular}{c} Sensor
    	%\\$x_k$ 
    	\end{tabular}}; 
		
		\node[minimum width = 0.0cm] (){};\&
		\node[block] (encoder) {\begin{tabular}{c} Quantizer/\\Encoder \end{tabular}}; 
		
		\node[minimum width = 0.0cm] (){};\&
		\node[block, fill=red!20, text=black ] (channel) {\begin{tabular}{c} Channel %\\ 
		\end{tabular}};
		
		\node[minimum width = 0cm] (){};\&
		\node[block] (decoder) {\begin{tabular}{c} Decoder 
		\end{tabular}}; 
		
		\node[minimum width = 0.0cm] (){};\&
		\node[block] (estimator) {\begin{tabular}{c} Estimator \\$\hat{x}_{k+d}$
		\end{tabular}};
		
    %\\
    %\&
    %\&
    %\&
    %\&
    %\node[block] (plant) {\begin{tabular}{c} Plant \end{tabular}}; 
		%\&
        \\
    };

%\draw [
%thick,
%decoration={
%	brace,
%	mirror,
%	raise=0.5cm
%},
%decorate
%] (encoder.south) -- (decoder.south);

\draw [decorate,decoration={brace,amplitude=10pt,mirror},xshift=-4pt,yshift=0pt]
($(encoder.south)-(10pt, 0pt)$) -- ($(decoder.south)+(10pt, 0pt)$) node [black,midway,xshift=-0cm, below=10pt] 
{Info. bits $r$, Latency $d$, Reliability $1-p_e$};
    	
    	\draw [connector] (plant) -- node [above] {}(sensor);
		\draw [connector] (sensor) -- node [above] {}(encoder);
		\draw [connector] (encoder) -- node [above] {}(channel);
		\draw [connector] (channel) -- node [above] {}(decoder);
		\draw [connector] (decoder) -- node [above] {}(estimator);
        
        %\draw [connector] (plant) -| node [left] {}(sensor);
        %\draw [connector] (actuator) |- node [right] {}(plant);

\end{tikzpicture}



==> timing.tex <==

\begin{tikzpicture}

%\begin{axis}[
%xmin=-3,   xmax=3,
%ymin=-3,   ymax=3,
%extra x ticks={-1,1},
%extra y ticks={-2,2},
%extra tick style={grid=major},
%]

\begin{axis}[
        clip bounding box=upper bound,
axis lines = middle,
    xmin=-1,xmax=23,
    ymin=-1.5,ymax=0.1,
      %axis x line=middle,
    axis y line=none, 
          %axis line style={draw=none},
    xlabel={\footnotesize Time steps (k)},
    x label style={at={(axis description cs:0.5,+1.0)}, anchor=south},
    %%xtick={-2,-1,...,3}
    %%minor tick num=4,
		xticklabel style={yshift=0.5ex, anchor=south},
		xtick={0, 1, ..., 22},
		xticklabels={0, ,,,, 5, ,,,,10,,,,,15,,,,,20},
		%xtick={0, 1, 2, 3,  4, 5, 6, 7, 8, 9, 10, 11 , 12, 13, 14, 15, 16, 17, 18, 19, 20},
		%xticklabels={,,},%{0, 1, 2, 3,  4, 5, 6, 7, 8, 9, 10, 11 , 12, 13, 14, 15, 16, 17, 18, 19, 20},
		%%xticklabels={0, ,,, ,5, 6, 7, 8, 9, 10, 11 , 12, 13, 14, 15, 16, 17, 18, 19, 20},
%
    %%xtick distance=0.1,
    %%xtick={0,1,2},
    %%ymin=0,
    %%ymax =1,
    %%ytick={},
    %y=0.5cm,
    %%x=10cm   
]
%\draw (axis cs:10,1) circle[radius=2];

\node (zerod) at (axis cs:0,-0.1) {};
\node (d) at (axis cs:4,-0.1) {};
\node (zeroT) at (axis cs:0,-.3) {};
\node (T) at (axis cs:9.9,-.3) {};

\node (Td) at (axis cs:10,-0.1) {};
\node (Tdd) at (axis cs:14,-0.1) {};

\node (TT) at (axis cs:10.1,-.3) {};
\node (TTT) at (axis cs:20,-.3) {};

\draw [<->]
(zerod.center) -- (d.center) node [black,midway,xshift=-0cm, below=0pt] 
{\footnotesize Latency d};

\draw [<->]
(zeroT.center) -- (T.center) node [black,midway,xshift=-0cm, below=0pt] 
{\footnotesize Sampling period T};

\draw [<->]
(Td.center) -- (Tdd.center) node [black,midway,xshift=-0cm, below=0pt] 
{\footnotesize Latency d};

\draw [<->]
(TT.center) -- (TTT.center) node [black,midway,xshift=-0cm, below=0pt] 
{\footnotesize Sampling period T};

%\draw [decorate,decoration={brace,amplitude=10pt,mirror},xshift=-4pt,yshift=0pt]
%(two) -- ($(three)$) node [black,midway,xshift=-0cm, below=10pt] 
%{Info};

\end{axis}


\end{tikzpicture}

